A Strong Composition Theorem for Junta Complexity and the Boosting of Property Testers

We prove a strong composition theorem for junta complexity and show how such theorems can be used to generically boost the performance of property testers. The $\varepsilon$-approximate junta complexity of a function $f$ is the smallest integer $r$ such that $f$ is $\varepsilon$-close to a function that depends only on $r$ variables. A strong composition theorem states that if $f$ has large $\varepsilon$-approximate junta complexity, then $g \circ f$ has even larger $\varepsilon'$-approximate junta complexity, even for $\varepsilon' \gg \varepsilon$. We develop a fairly complete understanding of this behavior, proving that the junta complexity of $g \circ f$ is characterized by that of $f$ along with the multivariate noise sensitivity of $g$. For the important case of symmetric functions $g$, we relate their multivariate noise sensitivity to the simpler and well-studied case of univariate noise sensitivity. We then show how strong composition theorems yield boosting algorithms for property testers: with a strong composition theorem for any class of functions, a large-distance tester for that class is immediately upgraded into one for small distances. Combining our contributions yields a booster for junta testers, and with it new implications for junta testing. This is the first boosting-type result in property testing, and we hope that the connection to composition theorems adds compelling motivation to the study of both topics.

==> Asymmetric.tex <==
\section{Asymmetrics vs symmetric noise stability}

\newcommand{\Ber}{\mathrm{Ber}}
\newcommand{\Bin}{\mathrm{Bin}}

First, we will restrict ourselves to symmetric $g$. Given a vector $\vec{\delta} = \delta_1, \ldots, \delta_k$, our goal is to make a statement of the following form:
\begin{align*}
    \NS_{\vec{\delta}}(g) = \NS_{\delta^\star}(g) \pm \eps
\end{align*}
where the rhs is symmetric noise stability, and
\begin{equation*}
    \delta^\star = \Ex_{i \in [k]}[\delta_i]\cdot (1 \pm 0.1).
\end{equation*}

\paragraph{Plan of attack}
Let $\bZ$ be defined as $\bZ \sim \sum_{i \in [k]} \Ber(\delta_i)$, indicating the distribution over number of input variables flipped. We wish to find a distribution over $\bp \in [0,1]$ such if we first sample a $p \sim \bp$ and then $\bZ' \sim \Bin(n, p)$, then the distribution of $\bZ'$ and $\bZ$ are identical. By writing out the moment generating functions, we get a relation for the first $k$ moments of $\bp$ that is both necessary and sufficient. The idea is that the values $\bp_i$ will correspond to the $\delta_i$ in a symmetric noise experiment.

Explicitly solving for the distribution over $\bp$ is difficult. Instead, we proceed in two steps: First, our plan is to show existentially that there is a distribution over $\bp$ that has the desired moments. Then, we show that \emph{any} such distribution concentrates around $ \Ex_{i \in [k]}[\delta_i]$, which will hopefully follow directly from the moment bounds.

Guy thinks without much thought that the goal is, for all $\ell \leq k$
\begin{align*}
    \Ex_{S \sim \binom{[k]}{\ell}}\left[\prod_{i \in S} \delta_i\right] = \Ex[\bp^\ell]
\end{align*}


To do for next time: figure out if 2-dim CLT approach works, and if so, how it compares with this more direct approach (more direct seems more likely to give sharper bounds?)



==> formulas.tex <==
\section{An XOR lemma for formulas}

\paragraph{Formulas.}{The formula complexity of a Boolean function $f:\bits^n\to\bits$ is $\Fm(f)\in\N$, the number of leaves in the smallest formula computing $f$. We write $\Fm_\eps(f)$ for the size of the smallest formula computing $f$ with error at most $\eps$ over the uniform distribution. Likewise, $\Fmr_\eps(f)$ is randomized formula complexity of computing $f$ to error $\eps$: the smallest expected size of any distribution over formulas computing $f$ to expected accuracy $\eps$. As with circuits, every function which is mildly hard to compute by formulas has a hardcore set. 

% \begin{theorem}[Impagliazzo's hardcore set lemma for formulas]
%     Suppose $f:\bits^n\to\bits$ is $\delta$-hard for size-$s$ formulas: $\Pr[f\neq F]>\delta$ for every formula $F$ with $|F|< s$. Then for all $\eps\in (0,1)$, there is a distribution $H$ of density $\Omega(\delta)$ such that $\Pr_H[f\neq  F]>1/2-\eps/2$ for all formulas $F$ of size $|F|\le s'=O(s\cdot \eps^2/\log(1/\delta))$.
% \end{theorem}

% \begin{theorem}[Impagliazzo's hardcore set lemma for general complexity measures]
%     Let $m:\bits^{2^n}\to\R$ be an arbitrary measure on $n$-bit Boolean functions. Suppose $f:\bits^n\to\bits$ is $\delta$-hard for measure-$s$: $\Pr[f\neq g]>\delta$ for all functions $g$ satisfying $m(g)\le s$. Then for all $\eps\in (0,1)$, there is a distribution $H$ of density $\delta$ such that $\Pr_H[f\neq g]>1/2-\eps/2$ for all $g$ satisfying $m(g)\le s'$ where $g_i:\bits^n\to\bits$ are fixed functions with $m(g_i)\le s$ and $k\le \eps^2/(12\log(2/\delta)))$.
% \end{theorem}

\begin{fact}
\label{fact:delta}
Any distribution over $\delta$ distributions is itself a $\delta$ distribution. 
\end{fact}

\begin{theorem}
    Let $m:\bits^{2^n}\to\R$ be an arbitrary measure on $n$-bit Boolean functions. Let $s'\in \N$ and $\eps,\delta\in (0,1)$ be such that for all density $\ge \delta$ distributions $H$, there exists some $g:\bits^n\to\bits$ with $m(g)\le s'$ satisfying
    $$
    \Prx_{\bx\sim H}[f(\bx)\neq g(\bx)]\le \frac{1}{2}-\frac{\eps}{2}.
    $$
    Then there exist $k\le 12\log(2/\delta)/\eps^2$ functions $g_1,\ldots,g_k:\bits^n\to\bits$ such that
    $$
    \Prx_{\bx\sim\mathcal{U}_n}[\textsc{MAJ}(g_1(\bx),\ldots,g_k(\bx))\neq f(\bx)]\le \delta
    $$
    and $m(g_i)\le s'$ for all $i\in [k]$. 
\end{theorem}


\begin{proof}
    Let $m,s',\eps,\delta,f$ be as in the theorem statement. Consider the matrix $M$ over $[0,1]$ whose rows are indexed by $\delta$ distributions $H$ over $\bits^n$ and whose columns are indexed by functions $g$ satisfying $m(g)\le s'$ and whose $(H,g)$th entry is $\Pr_H[f\neq g]$. Let $\alpha$ denote a distribution over $\delta$ distributions $H$ and let $\beta$ denote a distribution over functions $g$ with $m(g)\le s'$. Then by von Neumann's minimax theorem:
    \begin{equation}
    \label{eq:minimax}
    \max_\alpha\min_\beta \alpha^\top M\beta=\min_\beta \max_\alpha \alpha^\top M\beta.
    \end{equation}
    Let $\alpha$ be a fixed distribution over $\delta$ distributions and let $g^*$ satisfy $m(g^*)\le s'$ and $\Pr_\alpha[f\neq g^*]\le 1/2-\eps/2$. Such a $g^*$ must exist because $\alpha$ is itself a $\delta$ distribution by \Cref{fact:delta}. Then,
    \begin{align*}
        \min_\beta \alpha^\top M\beta &=\min_\beta\sum_i\beta_i\Prx_\alpha[f\neq g_i]\tag{$\alpha$ is a $\delta$ distribution}\\
        &\le \Prx_\alpha[f\neq g^*]\\
        &\le \frac{1}{2}-\frac{\eps}{2}.
    \end{align*}
    Let $\beta^*$ be a distribution over columns of $M$ that minimizes $\min_\beta \max_\alpha \alpha^\top M\beta$ and let $\alpha^*$ be a $\delta$ distribution that maximizes $\alpha^\top M\beta$. Then, we obtain
    \begin{align*}
        \frac{1}{2}-\frac{\eps}{2}&\ge \min_\beta \alpha^\top M\beta\\
        &=(\alpha^*)^\top M\beta^*\tag{\Cref{eq:minimax}}\\
        &=\Ex_{g\sim \beta^*}\left[\Prx_{\bx\sim\alpha^*}[f(\bx)\neq g(\bx)]\right].
    \end{align*}
    
\end{proof}
}


In this section, we prove the following XOR lemma which shows how $\Fm(f)$ scales with parity.

\begin{theorem}
    \label{thm:IHL-for-formulas}
    For all functions $f:\bits^n\to\bits$ and $\eps,\delta\in (0,1)$,
    $$
    \Fmr_{1/2-(1-\delta)^k-\eps}(f^{\oplus k})\ge \Omega\left(\frac{k\eps^2}{\log(1/\delta)}\cdot\Fmr_\delta(f)\right).
    $$
\end{theorem}

\begin{proof}
    Suppose for contradiction there is a formula $F$ computing $f^{\oplus k}$ with low error 
    $$
    \Pr[F\neq f^{\oplus k}]\le \frac{1}{2}-\eps-(1-\delta)^k
    $$
    and small size,
    $$
    |F|<k\frac{\eps^2}{\log(1/\delta)}\Fm_\delta(f).
    $$
    By the definition of $\Fm_\delta(f)$, $f$ is $\delta$-hard for size-$\Fm_\delta(f)$ formulas. Therefore, \Cref{thm:IHL-for-formulas} gives the existence of a hardcore distribution $H$ for $f$. We will obtain a contradiction by deriving a formula computing $f$ over the distribution $H$ with error at most $\eps$ and size strictly less than $\eps^2\Fm_\delta(f)/\log(1/\delta)$.

    We partition $\bits^{nk}$ into sets $R_\ell$ for $\ell\in\{1,\ldots,k\}$ where
    $$
    R_\ell\coloneqq\left\{(x_1,\ldots,x_k)\in(\bits^n)^k\mid \ell \text{ many }x_i \text{ are in }H\right\}.
    $$
    We then have
    \begin{align*}
        \Pr[F(\bx)=f^{\oplus k}(\bx)]=&\Pr[\bx\in R_0]\Pr[F=f^{\oplus k}\mid \bx\in R_0]+\\
        &\Pr[\bx\not\in R_0]\Pr[F=f^{\oplus k}\mid \bx\not\in R_0]\\
        \le& (1-\delta)^k+\Pr[\bx\not\in R_0]\Pr[F=f^{\oplus k}\mid \bx\not\in R_0]
    \end{align*}
    since a uniform random $x_i\in \bits^n$ is contained in $H$ with probability at least $\delta$. By our assumption on $F$:
    \begin{align*}
        \frac{3}{4}+\eps+(1-\delta)^k&\le \Pr[F\neq f^{\oplus k}]\\
        &\le (1-\delta)^k+\Pr[\bx\not\in R_0]\Pr[F=f^{\oplus k}\mid \bx\not\in R_0].
    \end{align*}
    By an averaging argument, there must be some fixed $\ell\neq 0$ such that
    $$
    \frac{3}{4}+\eps\le \Pr[F=f^{\oplus k}\mid \bx\in R_\ell].
    $$
    Let $R^{(i)}_{\ell-1}\sse R_{(\ell-1)}$ denote the set of strings $(x_1,\ldots,x_k)\in R_{(\ell-1)}$ where the $i$th block is not a hardcore block. For a string $y\in (\bits^n)^k$, $x\in \zo^n$ and $i\in[k]$, we write $y^{i\leftarrow x}\in (\bits^n)^k$ for the string obtained by inserting $x$ into the $i$th block of $y$. Therefore,
    \begin{align*}
        \Ex_{\bi\sim [k]}\left[\Ex_{\by\sim R^{(\bi)}_{\ell-1}}\left[\Prx_{\bx\sim H}\left[F(\by^{\bi\leftarrow \bx})\neq f^{\oplus k}(\by^{\bi\leftarrow \bx})\right]\right]\right]&= \Pr[F(\bx)\neq f^{\oplus k}(\bx)\mid \bx\in R_\ell].
    \end{align*}

    Also, for $i\in [k]$, we write $\size_i(F)\in\N$ to denote the number of leafs in $F$ from the $i$th input block. That is, $F$ contains $\size_i(F)$ many leaf variables $(x_i)_j$ for some $j\in [n]$. Since $\sum_{i\in [k]}\size_i(F)=|F|$, the expected size of a random block is small:
    $$
    \Ex_{\bi\in [k]}\left[\size_i(F)\right]=\frac{|F|}{k}.
    $$
    Therefore,
    \begin{align*}
        \Ex_{\bi\sim [k]}\left[\Ex_{\by\sim R^{(\bi)}_{\ell-1}}\left[\Prx_{\bx\sim H}\left[F(\by^{\bi\leftarrow \bx})\neq f^{\oplus k}(\by^{\bi\leftarrow \bx})\right]\right]\right]&\le\frac{1}{4}-\eps\\
        \Ex_{\bi\in [k]}\left[\size_i(F)\right]&\le \frac{\eps^2}{\log(1/\delta)}\cdot\Fm_\delta(f)
    \end{align*}
    and so by Markov's inequality there is some fixed $i^*$ such that
    \begin{align*}
        \Ex_{\by\sim R^{(\bi)}_{\ell-1}}\left[\Prx_{\bx\sim H}\left[F(\by^{i^*\leftarrow \bx})\neq f^{\oplus k}(\by^{i^*\leftarrow \bx})\right]\right]&\le \frac{1}{2}-2\eps\\
        \size_{i^*}(F)&\le \frac{2\eps^2}{\log(1/\delta)}\Fm_\delta(f).
    \end{align*}
    Finally, there is some fixed $y\in R^{(\bi)}_{\ell-1}$ such that
    $$
    \Prx_{\bx\sim H}\left[F(y^{i^*\leftarrow \bx})\neq f^{\oplus k}(y^{i^*\leftarrow \bx})\right]\le \frac{1}{2}-2\eps.
    $$
    By hardwiring the inputs outside of the $i^*$th block according to $y$, we obtain a formula $F'$ which computes $f^{\oplus k}(y^{i^*\leftarrow x})=b\oplus f(x)$ over the distribution $H$ where $b\in \bits$ is the fixed bit $b=\prod_{j\neq i}f(y_j)$. Moreover, after hardwiring these inputs, the size of the resulting formula is $|F'|=\size_{i^*}(F)\le 2\eps^2\Fm_\delta(f)/\log(1/\delta)$. We have therefore obtained a formula $F'$ satisfying:
    $$
    \Pr_H[f\neq F']<\frac{1}{2}-\frac{\eps}{2}\qquad \text{and}\qquad
        |F'|<\frac{\eps^2}{\log(1/\delta)}\cdot\Fm_\delta(f)
    $$
    which contradicts \Cref{thm:IHL-for-formulas}. 
\end{proof}



==> juntas.tex <==
\section{Intro}

Junta complexity is perhaps the most basic complexity measure of boolean functions. $k$-juntas are a subclass of depth-$k$ decision trees and width-$k$ DNFs, themselves considered to be extremely simple classes of functions, and special cases of more expressive classes such as formulas and circuits of size $2^k$. 

In this work we consider how junta complexity is affected by composition.  The zero-error case is completely obvious: if $f$ has zero-error junta complexity $k$ and $g$ has zero-error junta complexity $\ell$, then $g\circ f$ has junta complexity $k\ell$. 

Things become much more subtle when we consider approximate computation. Things that seem like they should be intuitively true are in fact false. 

Bigger picture: lots of interest in {\sl strong} composition theorems. Contrast with the famous Yao's XOR lemma for circuits, which is not strong.  We systematically build towards an understanding of strong composition theorems for expressive models (e.g.~circuits) by starting with the seemingly simplest complexity measure ever, junta complexity.  As we will see, even for juntas things get counterintuitive and technically interesting.  We conjecture that the broad connections to noise sensitivity that we establish in this work also hold for more expressive classes.  


Prior work on strong composition theorems:  Main thing to discuss here is Shaltiel counterexample for decision trees. Brody et al.~(aborts) and Drucker (only when inner noise rate sufficiently high), both arguably unsatisfactory. Our results show that Shaltiel's counterexample can be evaded for juntas instead of DTs. Discuss how our work suggests a more satisfactory resolution of Shaltiel's counterexample for DTs. 

\section{Strong composition theorems for junta complexity} 

\paragraph{Motivation.} If $f$ is hard to approximate with juntas, how hard is $g \circ f$ to approximate with juntas? Our answer: We show that the curve for $g \circ f$ is determined by that of $f$ and the (asymmetric) noise sensitivity of $g$. 

Furthermore, for symmetric functions $g$, we give even more information. If your global junta budget for $g \circ f$ is $R$, we show that essentially the best thing you can do is split the budget evenly among the $k$ blocks. 

\paragraph{Notation.} We write $\error_{f}(r)$ to denote the smallest error of a $r$-junta for $f$. We also write $J(f,\delta)$ to denote the smallest integer $r$ such that $\error(f,r) \leq \delta$. 


At a high level, we are interested in statements of the form, for $g: \zo^k \to \bits$,
\[ J(g \circ f,\eps) \ge k \cdot J(f,\delta) \]
where $\eps \gg \delta$ (ideally, $\eps = \frac1{2} - \textnormal{tiny})$.  In other words, ``strong" composition theorems for junta complexity.  An important special case will be $g = \XOR$.



\subsection{Noise sensitivity and stability} 

Given a vector $\delta \in [0, \frac{1}{2}]^k$ and $x \in \zo^k$, we define the notation $\by \overset{\delta}{\sim} x$ to indicate that $\by$ is formed by starting with $x$ and independently flipping each of the $i$ coordinates with probability $\delta_i$. For any $g: \zo^k \to \bits$, the noise sensitivity is defined
\begin{equation*}
    \NS_\delta(g) \coloneqq \Prx_{\bx \sim \zo^k, \by \overset{\delta}{\sim} \bx}[g(\bx) \neq g(\by)].
\end{equation*}
Similarly, the stability is defined as
\begin{equation*}
    \mathrm{Stab}_\delta(g) \coloneqq \Ex_{\bx \sim \zo^k, \by \overset{\delta}{\sim} \bx}[g(\bx) \cdot g(\by)].
\end{equation*}
It's easy to see that
\begin{align*}
    \Stab_\delta(g) = 1 - 2 \NS_\delta(g) \\
    \NS_\delta(g) = \frac{1}{2} \cdot (1 - \Stab_\delta(g))
\end{align*}


\subsection{Upper bound} 

\begin{claim} 
    Let $f: \zo^n \to \zo$ be balanced ($\E[f] = \frac{1}{2}$), and $\NS_\delta(g)$ refer to the noise sensitivity of $g$ at noise rate $\delta$. Then,
    \begin{align*}
        \error(g \circ f, R) \leq \NS_{2\cdot \error(f, \lfloor R/k \rfloor)}(g).
    \end{align*}

    More generally, for any $r_1 + \cdots + r_k = R$ where $r_i \geq 0$ for all $i \in [k]$, let $\delta(r_1, \ldots, r_k)$ be the vector $[\error(f, r_1), \ldots, \error(f, r_k)]$, using asymmetric noise sensitivity,
    \begin{equation*}        \error(g \circ f, R) \leq \NS_{2 \cdot \delta(r_1, \ldots, r_k)}(g) = \frac1{2} - \frac1{2} \Stab_{2\cdot \delta(r_1,\ldots,r_k)}(g). 
    \end{equation*}
\end{claim} 

A remark about the factor of $2$: this is because noise sensitivity is defined so that the probability of $1$ flipping to $0$ is the same as the probability of $0$ flipped into $1$.  However, the best junta approximator may make more errors on $1$-inputs than $0$-inputs or vice versa. 

\subsection{Lower bound} 


\begin{theorem} 
     Let $f: \zo^n \to \zo$ be balanced ($\E[f] = \frac{1}{2}$), for any vector of budgets $[r_1, \ldots, r_k]$,
     \begin{equation*}
         \error(g \circ f, [r_1, \ldots, r_k]) \geq \frac{1}{2} \cdot  \left(1 - \sqrt{\mathrm{Stab}_{\delta(r_1, \ldots, r_k)}(g)}\right)
     \end{equation*}
\end{theorem} 


\paragraph{Warm up.} $f$ balanced, uniform distribution Fourier expansion.  The real thing will require working over a carefully chosen product distribution. 

\begin{lemma}
    For any $g: \bits^k \to \bits$ and balanced $f: \bits^n \to \bits$ (i.e., $\E[f] = 0$), we view $g \circ f$ as a function of $nk$. Let $h:\bits^{nk} \to \bits$ be an arbitrary Junta depending on the coordinates $S = S_1 \cup S_2 \cup \cdots \cup S_k$ where $S_i$ are the relevant coordinates that are given as input to the $i^{\text{th}}$ copy of $f$. Then,\gnote{Below equation may not be exactly correct. Will edit it appropriately after the proof.}
    \begin{equation*}
        \Ex[(g\circ f)h] \leq \Stab_{\error(f,S_1)^2, \ldots, (\error(f, S_k^2)}(g)
    \end{equation*}
    where $\error(f,S_i)$ is the minimum error of a Junta on $S_i$ coordinates in approximating $f$.
\end{lemma}
\begin{proof}
    Throughout this proof, we will use $h^\star$ to refer to the best $S$-Junta approximator of $g \circ f$. Let $\alpha$ be a restriction to all the coordinates in $S$. Then, for any input $x$ consistent with $\alpha$,
    \begin{equation*}
        h^\star(x) = \sign\paren*{\Ex_{\bx}[g \circ f(\bx) \mid \bx\text{ is consistent with $\alpha$}]}
    \end{equation*}
    where $\sign(\cdot)$ rounds to $\bits$. Therefore, we can write
    \begin{align*}
        \Ex[(g \circ f)h^\star] &= \Ex_{\balpha}\bracket*{\sign\paren*{\Ex_{\bx}[g \circ f(\bx) \mid \bx\text{ is consistent with $\alpha$}]}\Ex_{\bx}[g \circ f(\bx) \mid \bx\text{ is consistent with $\alpha$}] } \\
        &=\Ex_{\balpha}\bracket*{\abs*{\Ex_{\bx}[g\circ f(\bx) \mid \bx\text{ is consistent with $\alpha$}]} }
    \end{align*}
    The above expectation is iterates over $\balpha$ being all possible restrictions of the $S$ coordinates. Each such restriction can be decomposed as $\balpha = \balpha_1 \cup \cdots \cup \balpha_k$ where $\balpha_i$ is a restriction to the coordinates within $S_i$.

    
    \gnote{Proof in progress}
\end{proof}



Note: this is cool because the junta approximator does not have to be of the form \[ g(\textnormal{$r_1$ junta},\ldots,\textnormal{$r_k$ junta}). \] 
Indeed, it does not even have to be of the form, for any function $h$, 
\[ h(\textnormal{$r_1$ junta},\ldots,\textnormal{$r_k$ junta}).\] 
\textbf{Example}: Here's a small example where the very best junta approximator does {\sl not} have the above form.

Let $g: \zo^2 \to \zo$ be the $\mathrm{AND}$ function. There are many choices for $f$, but let's do something like: $f: \zo^3 \times \zo^n \to \zo$ such that $\E_{\by}[f(x)]$ is "translate binary $x$ to integer and divide by $8$". This can be accomplished by making $f(x, \cdot)(y)$ approximately thresholds.

Also: can consider $g=\mathrm{AND}$. Let $f(x,y)=x_1\lor \ldots\lor x_n\lor (y_1\land\ldots\land y_m)$ for $m>n$. Then any budget of $r<n$, best $r$-junta for $f$ is $1$. But for $g(f^1,f^2)$ can do better (for just $r=n-1$):
\begin{itemize}
    \item query $x_1,\ldots,x_r$ in both $f^1$, $f^2$
    \item output $1$ if any of the variables are $1$
    \item otherwise, output $0$
\end{itemize}

Another choice for $f(x,y)$: Return an appropriately chosen threshold on $\sqrt{n} \cdot |x|_h + |y|_h$ where $n$ is the number of $y$ variables.

\textbf{The high level idea}: We want that after fixing the Junta variables, $\E[f]$ (where the expectation is taken over remaining variables) takes a spectrum of values depending on the choice of Junta variables. This way, when we compress that spectrum to a single bit, we lose the ability to accurately determine if $\E[f_1]\E[f_2] \geq 0.5$, which is what the optimal construction checks. 

\subsubsection{Corollary for symmetric functions} 

Here we'll apply Markov, and it comes down to understanding noise sensitivity of symmetric $g$'s at noise vector $(0,\ldots,0,\delta,\ldots,\delta)$.  By the symmetry of $g$, maybe this comes down to some sort of $2$-dim CLT.  We can hope that show that noise sensitivity of symmetric $g$ at such as noise vector is close to noise sensitivity at the symmetric noise rate $\delta/2$ for all coordinates. 

\begin{enumerate} 
\item From 10/25: It seems like the Annals of Probability $2$-dim CLT will work for us to get error $1/\sqrt{k}$. We should confirm this. 
\item As next steps: (1) give elementary proof that recovers $1/\sqrt{k}$ error: matching moments, Omer's stuff (2) get characterization with no error (like \Cref{eq:delta-star-equal}, for an appropriate $\delta^\star \approx \delta^{\mathrm{avg}}$).
\item Say something about nonsymmetric $g$'s. 
\item We believe that for any $\vec{\delta}$, we can find $k' \in \{k/2, k\}$ and $\delta^\star$ s.t. $\delta^\star k' = \delta^{\mathrm{avg}} k$ and
\begin{equation*}
    \NS_{\vec{\delta}}(g) = \Ex_{|\rho| = k - k'}\left[\NS_{\delta^\star}(g_\rho)\right].
\end{equation*}
The idea is to match moments of the flip distribution with a mixture of binomials, and then find a single representative.

\item Look into generalizations of symmetric functions (e.g. $d$-part symmetric). 
\end{enumerate} 

\subsection{For asymmetric functions} 

Let $\vec{\delta} \in [0, \frac{1}{2}]^k$ and define
\begin{equation*}
    \delta = \sum_{i \in [k]}\frac{\Inf_i(g) \delta_i(g) }{ \Inf(g) }
\end{equation*}
Here the hope is to show that 

\begin{equation*}
    \NS_{\vec{\delta}}(g) \approx \NS_{\delta}(g).
\end{equation*}
Note the left hand side is asymmetric, and the rhs is symmetric.

Or instead, want to show that for $\delta^\star$ the unique choice in $[0, \frac{1}{2}]$ s.t.,
\begin{equation}
    \label{eq:delta-star-equal}
    \NS_{\vec{\delta}}(g) = \NS_{\delta^\star}(g),
\end{equation}
we have that
\begin{equation*}
    \delta^\star = \Theta\left( \sum_{i \in [k]}\frac{\Inf_i(g) \delta_i(g) }{ \Inf(g) }\right)
\end{equation*}



\section{Implications for distribution-free junta testing}  

Boost $1/n$ error from SODA paper to $\Omega(1)$ error using XOR lemma. 


\begin{lemma}
For any function $f:\zo^n\to\zo$ balanced over $\mu$ satisfies
$$
J_{1/3}^{\mu^k}(\XOR\circ f^k)\ge \Omega(k \cdot J_{1/n}^\mu(f)).
$$
\end{lemma}


\begin{theorem}
    ``Tolerantly'' testing the class of $k$-juntas over $\zo^n$ with error $\eps=1/3$ requires time $n^{\Omega(k)}$
\end{theorem}



\section{Symmetric functions using the Fourier spectrum}

Hoped for statement:
for $\vec{\delta}\in [0,1/2]^k$, there exists a $1-2\delta^\star\in \left[\E[1-2\delta_i], \text{GM}(1-2\delta_i)\right]$ which satisfies
$$
\NS_{\vec{\delta}}(g)=\NS_{\delta^\star}(g).
$$
$\text{GM}(\cdot)$ denotes the geometric mean.

For our application, when $g$ is symmetric and $f$ is balanced can reduce to the case when $\delta_i\le 1/\sqrt{k}$ for all $i$. This is because the influence of $g$ must be at least $\sqrt{k}$ and so if any $\delta_i>1/\sqrt{k}$ can already lower bound the error. When all $\delta_i\le 1/\sqrt{k}$, we should get $\text{GM}(1-2\delta_i)\le \E[1-2\delta_i]^2$.

We'll try to understand the asymmetric noise stability of a symmetric function $g$ using the Fourier spectrum. First, we write

\begin{equation*}
        \Stab_{\vec{\delta}}(g) = \sum_{S \subseteq [k]} \left(\prod_{i \in S} (1 - 2\delta_i)\right) \hat{g}(S)^2.
\end{equation*}

If $g$ is symmetric, that $\hat{g}(S)$ is constant for all $S$ at the same level. We'll use
\begin{equation*}
    w_\ell = \sum_{|S| = \ell} \hat{g}(S)^2,
\end{equation*}
By symmetry, for any $S$ with $\ell$ elements, $\hat{g}(S)^2 = \frac{1}{\binom{k}{\ell}} w_{\ell}$. This allows us to write,

\begin{equation}
    \label{eq:stab-level}
    \Stab_{\vec{\delta}}(g) = \sum_{\ell \in [k]} \Ex_{\bS \sim \binom{[k]}{\ell}}\left[\prod_{\bi \in \bS} (1 - 2\delta_i)\right] w_{\ell}.
\end{equation}

Lets introduce some notation. For each level $\ell$,
$$h(\ell) = \Ex_{\bS \sim \binom{[k]}{\ell}}\left[\prod_{\bi \in \bS} (1 - 2\delta_i)\right]$$
and, $\delta(\ell)$ is the unique choice for $\delta \in (0,1)$ such that $(1 - 2\delta)^\ell = h(\ell)$. Then, by comparing \Cref{eq:stab-level} to the Fourier based expression for symmetric noise sensitivity, we have
\begin{equation*}
    \Stab_{\hat{\delta}}(g) = \Stab_{\delta^*}(g) \quad\quad\quad\text{where}\quad\quad\quad \delta^\star \in \left[\min_{\ell} \delta(\ell), \max_{\ell} \delta(\ell)\right].
\end{equation*}
This allows us to compare asymmetric noise stability to symmetric noise stability. We conjecture that $\delta(\ell)$ is monotone. When $\ell = 1$, we have that $\delta(\ell) = \Ex_{\bi \sim [k]}[\delta_{\bi}]$. When $\ell = k$, we get that
\begin{align*}
    \delta(k) = \frac{1}{2} \left(1 - \left(\prod_{i \in [k]}(1 - 2\delta_i)\right)^{1/k}\right).
\end{align*}
I think via some Taylor argument, we can show that $\delta(k) \leq \delta(1) + O(\max_{i \in [k]} \delta_i^2)$. If so, we get that,
\begin{equation*}
    \delta^\star \in \left[\Ex_{\bi}[\delta_{\bi}], \Ex_{\bi}[\delta_{\bi}] + O\left(\max_{i} \delta_i^2\right)\right].
\end{equation*}

Conjecture: If we assume that $\vec{\delta}$ has half $0$ half $2\delta$,
\begin{equation*}
    \NS_{\vec{\delta}}(g) =\NS_{\delta}(g) + O\left(\frac{\NS_{\delta}(g)^2 }{\sqrt{k}}\right).
\end{equation*}
To prove the above, we'll rely on the fact that symmetric functions that are not super biased have high noise sensitivity, so we only care about about the case where $\max_i \delta_i$ isn't already large. Note that $\NS_{\delta}(g) \in [0,\frac{1}{2}]$, so this is better than the CLT-based argument. It can also be much stronger in the regimes we care about, when the error is small.

\paragraph{Actually, we care about the easy side}
What we really care about showing is that $\delta^* \geq \Ex_{\bi}[\delta_{\bi}]$. This side is easier. We just need to show that,
\begin{equation*}
    h(\ell) \leq (1 - 2\Ex_{\bi}[\delta_{\bi}])^\ell.
\end{equation*}
We'll apply negative association (see this note by David \footnote{\url{https://www.cs.cmu.edu/~dwajc/notes/Negative\%20Association.pdf}}). Let $\alpha_i \coloneqq 1 - 2\delta_i$, and consider the random variables $\bz_1, \ldots, \bz_k$ which are a uniformly random permutation of $\alpha_1, \ldots, \alpha_k$. Since permutation distributions are negatively associated (Lemma 8 of David's note), we have that $\bz_1, \ldots, \bz_k$ are negatively associated. Then, define,
\begin{equation*}
    f_i(z_i) \coloneqq \begin{cases}
        z_i &\text{if }i \leq \ell\\
        1&\text{otherwise}.
    \end{cases}
\end{equation*} 

Applying negative association (Corollary 4 of David's note),
\begin{align*}
    \Ex_{\bz}\left[\prod_{i \in [n]} f_i(\bz_i)\right] &\leq \prod_{i \in [k]} \Ex_{\bz}\left[f_i(\bz_i)\right] \\
    &= \prod_{i \in [\ell]} \Ex_{\bz}\left[\bz_i\right]  \\
    &= (1 - 2\Ex_{\bi}[\delta_{\bi}])^\ell.
\end{align*}



\subsection{Some directions for asymmetric functions}


\paragraph{Understanding useful asymmetric function}. Look at functions like Talagrand's, or more simply, recursive majority. As in e.g. Mossel and O'Donnell, where they study the question in the setting of symmetric noise sensitivity \footnote{\url{https://www.cs.cmu.edu/~odonnell/papers/monotone.pdf}}. Understanding the asymmetric noise sensitivity of recursive majority should be very doable: if $1/\sqrt{n}$ fraction of coordinates are given noise rate $1/2$, does that suffice to guarantee at least constant noise sensitivity? 

\paragraph{Relationship between influence and noise sensitivity}
When $\vec{\delta}$ is close to $0$, we get that
\begin{equation*}
    \NS_{\vec{\delta}}(g) \approx \sum_{i \in [k]} \inf_i(g) \delta_i.
\end{equation*}
How long is this approximation good for? Perhaps, for ``reasonable" g we can replace it with a statement of the following form
\begin{align*}
     \NS_{\vec{\delta}}(g) \leq \sum_{i \in [k]} \inf_i(g) \delta_i\tag{always true} \\
     NS_{\vec{\delta}}(g) \geq \min\left(0.1, 0.1 \cdot  \sum_{i \in [k]} \inf_i(g)\delta_i\right) \tag{requires some reasonableness assumption on $g$.}
\end{align*}
For ``reasonable" $g$, we conjecture it is enough to compare the ``L2" influence vs regular influence. In particular, we want the following ratio to be bounded

\begin{equation*}
    \frac{\sum_{S} \hat{g}(S)^2 \cdot |S|^2}{\left(\sum_{S} \hat{g}(S)^2 \cdot |S|\right)^2} \leq C.
\end{equation*}


\newpage
